Well-Conditioned Polynomial Representations for Mathematical Handwriting Recognition

Previous work has made use of a parameterized plane curve polynomial representation for mathematical handwriting, with the polynomials represented in a Legendre or Legendre-Sobolev graded basis. This provides a compact geometric representation for the digital ink. Preliminary results have also been shown for Chebyshev and Chebyshev-Sobolev bases. This article explores the trade-offs between basis choice and polynomial degree to achieve accurate modeling with a low computational cost. To do this, we consider the condition number for polynomial evaluation in these bases and bound how the various inner products give norms for the variations between symbols.

==> IfExistsUseBBL.tex <==
% If this file exists, then the .bbl file is used instead of calling bibtex.
% It cannot be empty.   To force bibtex to run, rename this file to something else.
